Spectral reciprocity and matrix representations of unbounded operators

Motivated by potential theory on discrete spaces, we study a family of unbounded Hermitian operators in Hilbert space which generalize the usual graph-theoretic discrete Laplacian. These operators are discrete analogues of the classical conformal Laplacians and Hamiltonians from statistical mechanics. For an infinite discrete set $X$, we consider operators acting on Hilbert spaces of functions on $X$, and their representations as infinite matrices; the focus is on $\ell^2(X)$, and the energy space $\mathcal{H}_{\mathcal E}$. In particular, we prove that these operators are always essentially self-adjoint on $\ell^2(X)$, but may fail to be essentially self-adjoint on $\mathcal{H}_{\mathcal E}$. In the general case, we examine the von Neumann deficiency indices of these operators and explore their relevance in mathematical physics. Finally we study the spectra of the $\mathcal{H}_{\mathcal E}$ operators with the use of a new approximation scheme.

==> stoch-incompleteness.tex <==
%%!TEX root = SRAMO.tex

\subsection{Stochastic incompleteness and essentially self-adjoint operators}
\label{sec:Stochastic-incompleteness}

In this subsection, we consider implications for the heat equation when the Laplacian fails to be essentially self-adjoint. 
  Wojciechowski has recently given a characterization of stochastic completeness for certain classes of graphs; see \cite{Woj07,Woj09,Woj10}. Also, M. Keller and D. Lenz characterize stochastic completeness for regular Dirichlet forms on discrete sets in \cite{KellerLenz09, KellerLenz10}, and relate this to the stochastic completeness of graphs and subgraphs. Additionally, A. Weber has recently given a condition for stochastic completeness of graphs which may be understood as a weak curvature bound \cite{Web08}. We believe that this curvature bound implies Wojciechowski's criterion, which in turn implies \eqref{eqn:moderate-off-diagonal-growth}. Due to time constraints, this is left to a forthcoming paper.
  
  Stochastic incompleteness (see Definition~\ref{def:stochastic-completeness}) is closely related to the existence of nontrivial defect spaces of the Laplacian, although it should be understood that there is no implication either way (without further conditions). 
  Indeed, there exist examples of all four possible combinations of stochastic (in)completeness and essential (non)self-adjointness; see \cite{KellerLenz09}, especially \S4.

The reader familiar with Kato's description of the relationship between self-adjoint operators and quadratic forms \cite{Kat95} will see a parallel with the contents of the present section. However, the connection between semigroup theory and the operators $T_A$ discussed in \S\ref{sec:self-adjoint-operators-in-L2} (of which $\Lap_A$ is special cases) is not so transparent; especially with regard to the spectral theory of the semigroup operators in the context of $\ell^2(X)$. For example, see \cite{KF70, KL70, Phi61, Fe52, Fe59}, and their connections to Dirichlet forms \cite{FOT94, Ch01, RoSc95, HPS88}. 

\begin{defn}\label{def:contractive-semigroup}
  If $A$ is an infinite matrix defining a matrix Laplacian $\Lap_A$ as in Definition~\ref{def:matrix-Laplacian}, then the associated \emph{strongly continuous contractive semigroup} acting on $\ell^2(X)$ is defined by $S_t^{(A)} := e^{-t\Lap_A}$ via the spectral theorem. 
\end{defn}

\begin{prop}\label{thm:contractive-semigroup}
  The strongly continuous contractive semigroup $S_t = S_t^{(A)}$ satisfies the following: % properties:
  \begin{enumerate}
    \item $S_s S_t = S_{s+t}$, for $s,t \geq 0$, and $S_o = \id$.
    \item $\|S_t u\|_{\ell^2} \leq \|u\|_{\ell^2}$ for $t \geq 0$ and $u \in \ell^2(X)$.
    \item $\lim_{t \to 0} \|u - S_t u\|_{\ell^2} = 0$, for all $u \in \ell^2(X)$.
    \item $u \in \dom \Lap_A$ if and only if $\sup_{t \geq 0} \frac1t \|u - S_t u\|_{\ell^2} \leq \iy$, in which case $\Lap_A u = \lim_{t \to 0^+} \frac1t(u - S_t u)$.
  \end{enumerate}
\end{prop}

%We continue to suppress the dependence on $A$ for ease of notation, and 
From now on, we write $S_t = S_t^{(A)}$, $p_t(x,y) = p_t^{(A)}(x,y)$ and $\Lap = \Lap_A$.

\begin{defn}\label{def:heat-kernel}
  The \emph{heat kernel} is 
  %\linenopax
  %\begin{align}\label{eqn:heat-kernel}
  $  p_t(x,y) := \la \gd_x, S_t \gd_y \ra_{\ell^2}. $
  %\end{align}
\end{defn}

\begin{remark}[Positivity of the kernel]
  \label{rem:positivity-of-the-kernel}
  For researchers working in potential theory and harmonic analysis, it is natural to expect that $p_t(x,y) \geq 0$, especially in light of the heat kernel's interpretation in terms of transition probabilities. However, for the more general case of an operator given by a positive semidefinite matrix $A$, the associated semigroup has matrix entries defined by $e^{-tA}$ in the sense that \smash{$p_t(x,y) = \ipH[\ell^2]{\gd_x, S_t \gd_y} = [e^{-tA}]_{x,y}$}. In general, it is not the case that the kernel $p_t(x,y)$ is nonnegative. For example, this fails for the Heisenberg matrices (matrix representations of the position and momentum operators in quantum mechanics) and various functions of them. % discussed in \S\ref{sec:Unbounded-operators-and-banded-matrices}; see Example~\ref{exm:negative-kernels}. 
  We expect that under the assumption that $\|e^{-tA}\| \leq 1$ for all $t > 0$, the conditions of Definition~\ref{def:matrix-Laplacian} are sufficient to ensure 
  \linenopax
  \begin{align}\label{eqn:p_t(x,y)>0}
    p_t(x,y) = \ipH[\ell^2]{\gd_x, e^{-tA} \gd_y} \geq 0,  \qq \text{for all } x,y \in X \text{ and } t>0,
  \end{align}
  and perhaps this is even equivalent to Definition~\ref{def:matrix-Laplacian}. If \eqref{eqn:p_t(x,y)>0} holds, then it follows that for fixed $x$ and $t$, $\sum_{y \in X} p_t(x,y)$, and hence the probabilistic interpretation carries through. To see this, let $\{F_n\}$ be any exhaustion of $X$ by finite sets as in Definition~\ref{def:exhaustion-of-X}, and note that 
  \linenopax
  \begin{align*}%\label{eqn:}
    \sum_{y \in F_n} p_t(x,y) 
    = \sum_{y \in F_n} \ipH[\ell^2]{e^{-tA}\gd_x,\gd_y}
    \leq 1
  \end{align*}
  by Schwarz's inequality and Bessel's inequality, whence Fatou's lemma gives
  \linenopax
  \begin{align}\label{eqn:sum(p_t(x,y))<1}
    \sum_{y \in X} p_t(x,y) 
    \leq \liminf_{n \to \iy} \sum_{y \in F_n} p_t(x,y)
    \leq 1.
  \end{align}
  Note that there is a massive literature on the situation where \eqref{eqn:p_t(x,y)>0} is satisfied. Consequently, we will leave further discussion of that topic to the experts.
\end{remark}

\begin{defn}\label{def:stochastic-completeness}
  When $p_t(x,y)$ is interpreted probabilistically, so that \eqref{eqn:p_t(x,y)>0} and \eqref{eqn:sum(p_t(x,y))<1} hold, one says that the system is \emph{stochastically complete} iff equality holds in \eqref{eqn:sum(p_t(x,y))<1}.%; see Remark~\ref{rem:curvature-estimates}.
\end{defn}

The following result appears in more extensive form in \cite[Thm.~3.1.3]{Woj07}, and has been extended to the more general setting of Dirichlet forms and symmetric Markov process in \cite[Thm.~1]{KellerLenz09} (where the presence of a potential or ``killing term'' is also taken into account).

\begin{theorem}[{$\negsp[4]$\cite[Thm.~3.1.3]{Woj07}}]
  \label{thm:stochastic-completeness}
  The following statements are equivalent:
  \begin{enumerate}%[(1)]
    \item The heat kernel is stochastically incomplete.
    \item There exists a nonzero bounded solution to $\Lap u(x,t) + \frac{\del u}{\del t}(x,t) = 0$ with $u(x,0) \equiv 0$.
    \item There exists a nonzero bounded function $v$ on $X$ such that $\Lap v(x) = \gl v(x)$ at each $x \in X$, for some $\gl < 0$.
  \end{enumerate}%[(1)]
\end{theorem}

The second item in Theorem~\ref{thm:stochastic-completeness} explains the nomenclature ``stochastically incomplete''. The third shows the relation to essential self-adjointness of \Lap: if \Lap acts on the Hilbert space \bH and $v\in \bH$ satisfies the Hilbert space identity $\Lap v = \gl v$ with $\gl < 0$, then \Lap is not essentially self-adjoint. Theorem~\ref{thm:stochastic-completeness} is generalized in a forthcoming paper by Keller and Wojciechowski; \cite{KellerWojciechowski10}.

The following results appeared in \cite[Cor.~3.3.1 and Thm.~3.3.4]{Woj07} and \cite[\S4]{Woj10} and pertain to a graph $G$. The notation $m(x)$ indicates the number of edges incident upon the vertex $x$. A \emph{tree} is a graph $T$ which contains no cycles, and tree is \emph {spherically symmetric} iff $m(x)$ depends only on the distance $r=d(x,x_0)$, where $d(x,y)$ is the  number of edges between $x$ and $y$. For spherically symmetric trees, denote $m(r) = m(x)$.

\begin{theorem}[Wojciechowski's Criteria]\label{thm:Radek's-criteria}
  If $T$ is a spherically symmetric tree, then $T$ is stochastically complete (i.e., the heat kernel on $T$ is stochastically complete) iff
  \linenopax
  \begin{align}\label{eqn:Radek's-criteria1}
    \sum_{r=0}^\iy m(r)^{-1} = \iy.
  \end{align}
  If $G$ is any graph with a vertex $x_0$ such that $M(r) := \max\{m(x) \suth d(x,x_0) =r\}$ satisfies
  \linenopax
  \begin{align}\label{eqn:Radek's-criteria2}
    \sum_{r=0}^\iy M(r)^{-1} = \iy.
  \end{align}
  then $G$ is stochastically complete. 
\end{theorem}

%\subsection{Unbounded operators and banded matrices}
%\label{sec:Unbounded-operators-and-banded-matrices}


\begin{defn}\label{def:banded-matrix}
  An infinite matrix $A = (a_{x,y})_{x,y \in X}$ is \emph{banded} iff each row and each column has only finitely many nonzero entries. If there is an integer $b$ such that no row or column of $A$ has more than $b$ entries, then $A$ is \emph{uniformly banded}. If $b$ is the least upper bound on the row/column size of a uniformly banded matrix, then it is called the \emph{band width} of $A$.
\end{defn}

\begin{remark}\label{rem:banded}
   In general, it is difficult to determine operator-theoretic and spectral-theoretic properties of operators in Hilbert space from a representation of the operators in the form of an infinite matrix. This was noted by von Neumann in \cite{vN43} and \cite{vN51}. However, restriction to the class of banded (infinite) matrices allows one to obtain many explicit results. Banded matrices occur frequently in mathematical physics, and include Jacobi matrices, Heisenberg's position and momentum matrics $P,Q$, and polynomials in $P$ and $Q$. In the context of graphs and networks, banded matrices arise as graph Laplacians (or incidence matrices) for examples where each vertex has only finitely many neighbours.
\end{remark}


\begin{defn}\label{def:banded-operator}
  Let $T$ be a Hermitian operator with a dense domain \sD in a Hilbert space \bH. We say that $T$ is a \emph{banded operator} if there is a nested family
  \linenopax
  \begin{align*}%\label{eqn:}
    \bH_1 \ci \bH_2 \ci \dots \ci \bH_n \ci \bH_{n+1} \ci \dots
  \end{align*}
  of finite-dimensional subspaces in \bH such that the following three conditions hold:
  \linenopax
  \begin{enumerate}[(i)]
    \item $\bH_n \ci \sD \label{eqn:H_k-in-D}$, 
    \item for each $n$, there is an $m > n$ such that $T\bH_n \ci \bH_{m}$ \label{eqn:AH_k-in-H_k+1}, and
    \item $\bigcup\nolimits_{n=1}^\iy \bH_n$ is dense in \bH. 
  \end{enumerate}
\end{defn}

We leave the proof of the following lemma as an exercise for the reader.
\begin{lemma}\label{thm:bandedness-equivalence}
  If $T$ is a banded operator in the sense of Definition~\ref{def:banded-operator}, then there exists an onb of \bH which is contained in \sD, and in this basis, the matrix representation $A_T$ of $T$ is a banded matrix in the sense of Definition~\ref{def:banded-matrix}. Conversely, if $A$ is a banded matrix, then multiplication by $A$ defines an operator $T_A$ which is banded.
\end{lemma}


\begin{defn}\label{def:moderate-off-diagonal-growth}
  Let $T$ be banded, so that $\bH$ and $\{\bH_k\}_{k=1}^\iy$ are as in Definition~\ref{def:banded-operator}, and for each $k=1,2,\dots$, let $P_k$ be the projection onto $\bH_k$.  Then $T$ is of \emph{moderate off-diagonal growth} iff the operator norm of the sequence $\{P_k^\perp T P_k\}_{k=1}^\iy$ satisfies
  \linenopax
  \begin{align}\label{eqn:moderate-off-diagonal-growth}
    \sum_{k=1}^\iy \left\|P_k^\perp T P_k\right\|^{-1} = \iy.
  \end{align}
\end{defn}

\begin{theorem}[{\cite{Jor77}}]
  \label{thm:moderate-off-diagonal growth-implies-ess-self-adjoint}
  Suppose a Hermitian operator $T$ is of moderate off-diagonal growth. Then it is essentially self-adjoint.
\end{theorem}

We will address the comparison of \eqref{eqn:Radek's-criteria2} and \eqref{eqn:moderate-off-diagonal-growth} in another paper.

\begin{comment}\label{rem:Jacobi-matrix}
  If an operator $T$ in $\ell^2(\bZ_+)$ is given by a Jacobi matrix $A$, and if 
  \linenopax
  \begin{align*}%\label{eqn:}
    \bH_k := \spn\{\gd_o,\gd_1,\dots,\gd_k\}
  \end{align*}
  and $P_k$ is the projection to $\bH_k$, then 
  \linenopax
  \begin{align*}%\label{eqn:}
    \left\|P_k^\perp T P_k\right\| = |b_k|,
  \end{align*}
  where $b=(b_1,b_2,\dots)$ is the complex sequence describing the off-diagonals, as in \eqref{eqn:Jacobi-matrix} of Definition~\ref{def:Jacobi-matrix}
  As a result, we see that the conclusion in Lemma~\ref{thm:Jacobi-selfadjointness}a follows from Theorem~\ref{thm:moderate-off-diagonal growth-implies-ess-self-adjoint}.
\end{comment}




